E-PINNs: Epistemic Physics-Informed Neural Networks

Physics-informed neural networks (PINNs) have demonstrated promise as a framework for solving forward and inverse problems involving partial differential equations. Despite recent progress in the field, it remains challenging to quantify uncertainty in these networks. While techniques such as Bayesian PINNs (B-PINNs) provide a principled approach to capturing epistemic uncertainty through Bayesian inference, they can be computationally expensive for large-scale applications. In this work, we propose Epistemic Physics-Informed Neural Networks (E-PINNs), a framework that uses a small network, the epinet, to efficiently quantify epistemic uncertainty in PINNs. The proposed approach works as an add-on to existing, pre-trained PINNs with a small computational overhead. We demonstrate the applicability of the proposed framework in various test cases and compare the results with B-PINNs using Hamiltonian Monte Carlo (HMC) posterior estimation and dropout-equipped PINNs (Dropout-PINNs). In our experiments, E-PINNs achieve calibrated coverage with competitive sharpness at substantially lower cost. We demonstrate that when B-PINNs produce narrower bands, they under-cover in our tests. E-PINNs also show better calibration than Dropout-PINNs in these examples, indicating a favorable accuracy-efficiency trade-off.

==> notes.tex <==






% \section{Appendix: Aleatoric Uncertainty Estimation Details}
% \label{sec:appendix_b_aleatoric}

% This appendix details the practical estimation of the average aleatoric variance component, $E_z[\text{Var}[u_\theta(x, z)|z]]$. This component is approximated by assuming a homoscedastic aleatoric variance, $\sigma_A^2$, which relates to the `noise_level` parameter (representing a standard deviation $\sigma_{\text{noise}}$) introduced during the training phase. The interpretation of how $\sigma_A^2$ connects to $(\texttt{noise\_level})^2$ varies with the problem type.

% \subsection{Aleatoric Uncertainty in Function Regression (ENN)}
% For direct function regression problems, where the physics-informed component is absent, we refer to the model as an Epistemic Neural Network (ENN). The ENN $u_\theta(x,z)$ is trained to approximate a target function $u_{\text{true}}(x)$. If noise is added directly to the observations of this function, the network is trained on noisy targets $y(x) = u_{\text{true}}(x) + \epsilon_u(x)$, where $\epsilon_u(x) \sim \mathcal{N}(0, \sigma_{\text{noise}}^2)$. In this scenario, the `noise_level` parameter directly corresponds to $\sigma_{\text{noise}}$.

% The output of the ENN for a fixed $z$, $u_{\theta, \text{out}}(x,z)$ (interpreted as $E[u_\theta(x,z)|z]$), estimates $u_{\text{true}}(x)$. The variance of the observation noise, $\sigma_{\text{noise}}^2$, directly represents the aleatoric variance in the output space of $u_\theta$. Therefore, for function regression with an ENN:
% \begin{align}
% \sigma_A^2 \approx \sigma_{\text{noise}}^2 = (\texttt{noise\_level})^2
% \end{align}
% This approximation is direct because the training noise is defined in the same space as the network's output.

% \subsection{Aleatoric Uncertainty in PDE Problems (E-PINN)}
% For PDE problems of the form $\mathcal{N}_x(u; \lambda) = f(x)$, the `noise_level` ($\sigma_{\text{noise}}$) introduced during E-PINN training is typically associated with the source term $f(x)$ or the overall PDE residual. The E-PINN is trained such that its prediction $u_\theta(x,z)$ satisfies $\mathcal{N}_x(u_\theta(x,z); \lambda) \approx f(x) + \epsilon_f(x)$, where $\epsilon_f(x) \sim \mathcal{N}(0, \sigma_{\text{noise}}^2)$.

% The solution to the PDE is $u(x) = \mathcal{N}_x^{-1}(f(x); \lambda)$, where $\mathcal{N}_x^{-1}$ denotes the inverse (solution) operator. Noise $\epsilon_f(x)$ in the source term propagates through this inverse operator, inducing an aleatoric variance in the solution $u_\theta(x,z)$. The precise relationship between $\text{Var}[\epsilon_f(x)] = \sigma_{\text{noise}}^2$ and the resultant aleatoric variance in the solution, $\sigma_A^2 = \text{Var}[u_\theta(x,z)|z]$, depends on the characteristics of $\mathcal{N}_x^{-1}$. This propagation can be complex and may not be uniform across the domain $x$ \cite{sullivan2015introduction}.

% In the absence of a detailed error propagation analysis, a common simplifying approximation is to assume that the aleatoric variance in the solution space, $\sigma_A^2$, can be directly represented by the variance of the noise applied to the source term or residual during training:
% \begin{align}
% \sigma_A^2 \approx \sigma_{\text{noise}}^2 = (\texttt{noise\_level})^2
% \end{align}
% It is important to recognize this as an approximation for PDE problems. The actual aleatoric variance in the solution might differ. A more rigorous approach would involve deriving the propagated variance or modifying the E-PINN architecture to explicitly predict a heteroscedastic aleatoric variance, $\sigma_A^2(x,z)$, typically by training with a Gaussian Negative Log-Likelihood loss.

% \subsection{Practical Estimation of Total Variance}
% Given these considerations, the total predictive variance in our implementation (which does not explicitly predict heteroscedastic aleatoric variance) is estimated as:
% \begin{align}
% \text{Var}[u_\theta(x, z)] \approx \text{Var}_z[u_{\theta, \text{out}}(x,z)] + (\texttt{noise\_level})^2
% \end{align}
% where $u_{\theta, \text{out}}(x,z)$ represents the mean output of the ENN/E-PINN for a given $z$, $\text{Var}_z[u_{\theta, \text{out}}(x,z)]$ is its variance across different epistemic samples $z$ (the epistemic component), and $(\texttt{noise\_level})^2$ is the approximated average aleatoric variance component.

